An Evaluation of Anomaly Detection and Diagnosis in Multivariate Time Series

Several techniques for multivariate time series anomaly detection have been proposed recently, but a systematic comparison on a common set of datasets and metrics is lacking. This paper presents a systematic and comprehensive evaluation of unsupervised and semi-supervised deep-learning based methods for anomaly detection and diagnosis on multivariate time series data from cyberphysical systems. Unlike previous works, we vary the model and post-processing of model errors, i.e. the scoring functions independently of each other, through a grid of 10 models and 4 scoring functions, comparing these variants to state of the art methods. In time-series anomaly detection, detecting anomalous events is more important than detecting individual anomalous time-points. Through experiments, we find that the existing evaluation metrics either do not take events into account, or cannot distinguish between a good detector and trivial detectors, such as a random or an all-positive detector. We propose a new metric to overcome these drawbacks, namely, the composite F-score ($Fc_1$), for evaluating time-series anomaly detection. Our study highlights that dynamic scoring functions work much better than static ones for multivariate time series anomaly detection, and the choice of scoring functions often matters more than the choice of the underlying model. We also find that a simple, channel-wise model - the Univariate Fully-Connected Auto-Encoder, with the dynamic Gaussian scoring function emerges as a winning candidate for both anomaly detection and diagnosis, beating state of the art algorithms.

==> files/10_summary_of_changes.tex <==
% \section{Summary of changes (Round 2)}

% We thank the reviewers for additional constructive feedback that has helped us improve the clarity of the paper. 

% \subsection{Reviewer 1}

% \textbf{Reviewer}: I think the main take-away message of the paper can still be described more clearly. 

% \textbf{Authors}: To improve clarity, we have separated a part of the abstract into a new paragraph that reads as the following: 

% \agcomment{Our study highlights that dynamic scoring functions work much better than static ones for multivariate time series anomaly detection, and the choice of scoring functions often matters more than the choice of the underlying model. We also find that a simple, channel-wise model - the Univariate Fully-Connected Auto-Encoder, with the dynamic Gaussian scoring function emerges as a winning candidate for both anomaly detection and diagnosis, beating state of the art algorithms.}

% In addition, we have italicized a sentence in each of the bullet points under section \ref{sec:contributions} Contributions that conveys the key message for that bullet. 

% ----------------

% \textbf{Reviewer}: "Thus we find that the existing evaluation metrics either do not take events into account, or are not robust..." What is meant with "robust"? This is never defined explicitly, so this claim is vague and difficult to assess (e.g., robustness to noise, sample size, class imbalance...?).

% \textbf{Authors}: By "robust", we meant robustness to naive detectors such as random detection or classifying everything as an anomaly. 

% For clarity, we have reworded ‘or are not robust…’ to \agcomment{or cannot distinguish between a good detector and trivial  detectors,  such  as  a  random  or  all-positive  detector} in the abstract. 

% ----------------

% \textbf{Reviewer}: - "CPS unlike many distance-based and pattern-based techniques that require the entire time-series..." -- Maybe reword this as "anomaly detection algorithms that explicitly learn a model and algorithms that do not"

% \textbf{Authors}: Some algorithms that do not learn an explicit model can still work in a streaming scenario, although this is an exception rather than the rule. But we cannot make a blanket statement about all non-model algorithms, thus limit ourselves to saying ‘many distance-based and pattern-based techniques’ in the sentence below. 

% To avoid confusion, we have reworded in the following manner:

% (Original) 
% ‘(b) fast inference and applicability to streaming time-series typical in CPS unlike many distance-based and pattern-based techniques that require the entire time-series (i.e. both training and test data) during inference’ 

% (Reworded)
% \agcomment{(b) fast inference and applicability to streaming time-series typical in CPS unlike many distance-based and pattern-based techniques that are not applicable to streaming time-series, as they require both training and test data during inference}

% ----------------

% \textbf{Reviewer}: "We evaluate semisupervised and unsupervised deep anomaly detection techniques for MVTS..." -- All the training data are assumed to be anomaly-free. In practice this means that somebody has checked the data and removed (potential) anomalous events from the training data. I'd consider this a fully semi-supervised setting. In my mind, the paper does not conduct unsupervised anomaly detection.

% \textbf{Authors}: The observation is correct - we evaluate only in the semi-supervised setting but some of the algorithms, such as DAGMM and OC-SVM - are unsupervised algorithms, that can also be used in the semi-supervised setting. 

% Thus to clarify further, we have removed the word unsupervised in the sentence quoted above. Furthermore, we have added notes to the descriptions of DAGMM and OC-SVM instead, like so: 

% (Original) 
% DAGMM, an algorithm for unsupervised multivariate anomaly detection where an AE is...

% (Reworded)
% \agcomment{DAGMM, an algorithm for unsupervised multivariate anomaly detection (that can also be used in the semi-supervised setting) where an AE is...}

% (Original) 
% OC-SVM, a classic shallow technique for one-class classification...
	
% (Reworded)
% \agcomment{OC-SVM, a classic shallow technique for unsupervised anomaly detection via one-class classification...}

% ----------------

% \textbf{Reviewer}: Table 1: "Dims, m" -- terminology is a bit confusing as you use dims in the table and channels in the text.

% \textbf{Authors}: Replaced Dims with \agcomment{Channels} in Table 1

% ----------------

% \textbf{Reviewer}: Table 1: "Num events" -- Rename to "Avg num events per entity", that also clarifies why there are non-discrete numbers in this column.

% \textbf{Authors}: This was previously mentioned only in the table caption. For clarity, the column ‘Num events’ has now been renamed to \agcomment{Average num events}. The prefix \agcomment{Average} has been added to all columns where this applies (train length, test length, \% anomalies and num events). 

% We have also reworded the caption:

% (Original) Train length, test length, \% anomalies and num events are averaged over entities for multi-entity datasets. 

% (Reworded) \agcomment{Averaging is done over entities.}

% ----------------

% \textbf{Reviewer}: The Gaussian scoring functions fit a Gaussian distribution to the training errors. Then, anomalies are identified as points with an error that is uncommon under this Gaussian distribution. Does that also mean that very low reconstruction errors are considered anomalous? I assume that you use the cdf instead of pdf to avoid exactly this, but that is not clear from the text.

% \textbf{Authors}: The phrase ‘since $-\log (1 - cdf)$ is  monotonically  increasing with  error’ was meant to explain this. For clarity, this paragraph has now been reworded: 

% (Original) Similar to \cite{malhotra2016lstm}, we fit a Gaussian distribution, to the training errors and use the probability as an estimate of the anomaly score. Here we choose natural log of the complement of the cumulative distribution function (cdf), $-\log (1 - cdf)$ as $f_{trans}$ rather than $-\log pdf$ (pdf: probability distribution function) since $-\log (1 - cdf)$ is monotonically increasing with error. 

% (Reworded) 
% \agcomment{Similar to \cite{malhotra2016lstm}, we fit a Gaussian distribution to the training errors and design a score based on the fitted distribution. We note that directly using the probability distribution function (pdf) as in $-\log pdf$ would give points at both tails of the distribution high scores. In particular, this means that even points with very low reconstruction errors will be classified as being anomalous. To avoid this, we instead develop a score based on the cumulative distribution function (cdf): $-\log (1 - cdf)$, that increases monotonically with reconstruction error as $f_{trans}$.}

% ----------------

% \textbf{Reviewer}: The Gauss-D-K scoring function would benefit from a couple of sentences explaining the intuition. Later in the paper, the authors state "Gauss-D-K performs better overall than Gauss-D by amplifying anomaly scores from multiple channels responding to the same anomaly, even if they respond at slightly different times." This suggests that the Gauss-D-K scoring function takes into account the errors of multiple timestamps and not a single timestamp slice across all channels? This should be clarified.

% \textbf{Authors}: The Gauss-D-K scoring function refers to Gaussian kernel convolution applied on top of Gauss-D, proposed by \cite{ahmad2017numenta} as a means to model the interdependency between channels with random temporal delays built in.

% (Reworded) \agcomment{This scoring function refers to Gaussian kernel convolution applied on top of Gauss-D\cite{ahmad2017numenta}. The smoothing of the score before aggregation can potentially amplify the total anomaly score even when multiple channels respond to an anomaly at slightly different times, unlike the previous three scoring functions.}

% ----------------

% \textbf{Reviewer}: "A validation set with anomalies could be used to set a static threshold [7], [9] but we do not assume the availability of such a validation set in our study." However, later the authors do hyperparameter tuning on the test set (e.g., selecting the best e-value for the tail-p threshold). This defeats a bit the purpose as it would then be better to assume (for the sake of the experiment) to have access to a validation set and test on a separate test set (instead of tuning on the test set).

% \textbf{Authors}: Indeed, having a validation set representative of anomalies to be encountered during testing would have been ideal to tune the tail probability threshold. However, there were two main challenges in partitioning our test set to obtain a validation set with anomalies: 
% \begin{itemize}
%     \item there are only a small number of test examples in each dataset, meaning that the validation set may not be sufficient to tune the threshold, and, 
%     \item Even if we designated an initial percent of the test set as a validation set, the example anomalies may not be representative of test anomalies.
% \end{itemize}

% In practice, the tail probability could be tuned during testing based on an ongoing evaluation of precision and recall, without having to tune the rest of the algorithm. Alternatively, practitioners in the industry may be able to come up with a validation set that is indeed representative of test-set anomalies. 

% In the absence of a representative validation set, however, our goal in the evaluation was to understand an upper-bound on the performance that can be achieved by tuning the threshold; we note that this practice is common in the literature \cite{su2019omni, audibert2020usad, li2019mad}.

% ----------------

% \textbf{Reviewer}: Fig 2: the Fc1 score for y3 is worse than that of the random detector and the all positive detector. This indicates that the Fc1 measure still has some flaws, as the result of y3 is quite good: all events are detected with only 2 false alarms (e.g., compared to the random detector which has many more false alarms, yet a higher Fc1 score). Maybe the authors can share some insight into why this is happening?

% \textbf{Authors}: Each of y1, y2 and y3 have eventwise recall of 1 and a substantial number of false positives (FPs). The difference lies only in the fraction of FPs and their distribution over time. The Fc1 scores of each of these detectors is quite low (Fc1<0.5) based on the time-wise precision, which only considers the fraction of FPs but ignores their distribution. 

% Ignoring the distribution of FPs, and consequently, ignoring ‘events’ in counting FPs may be thought of as a compromise in the metric to avoid a much bigger flaw - if we took events into account for precision as well, the all positive detector, y2 would become a perfect detector. This is because it has effectively only 1 event which is a true positive. This is the flaw with the event-wise F1 score \cite{hundman2018detecting} which does exactly that. 

% Lastly, we do not intend to use our metric to distinguish among poor detectors, rather to distinguish among good detectors. No metric is absolutely perfect, and also depends on what behavior one might consider desirable for a certain problem. We believe that for our evaluation, Fc1 score makes the most sense as it avoids the pitfalls of other metrics as explained in the paper. 

% \subsection{Reviewer 2}

% \textbf{Reviewer}: Because this is an experimental paper, I suggest the authors make a repository for all the code and settings.

% \textbf{Authors}: The code will be shared at this link upon paper acceptance: https://github.com/astha-chem/mvts-ano-eval
% We have included the following line under section 1A Contributions : \agcomment{The code will be released at \url{https://github.com/astha-chem/mvts-ano-eval}, upon paper acceptance.}


% \subsection{Reviewer 3}

% \textbf{Reviewer}: One minor suggestion is to enlarge the plots in Figure 4 as they are too small to read.

% \textbf{Authors}: In order to improve the readability of this figure within the constraints of space, we have enlarged the figure but broken it down into 2 parts. We now show 4 datasets in the main manuscript Figure 4 and refer the interested reader to the plots for additional datasets in the SI Fig S6. 

% \subsection{Summary of changes}
% \begin{itemize}
%     \item Some rewording in abstract. Abstract is now broken into two parts
%     \item Small addition to bullet 1 under section \ref{sec:contributions}, Contributions. 1 sentence has been italicized for each bullet point. 
%     \item Added link to the webpage where code will be shared upon acceptance in section \ref{sec:contributions} Contributions. 
%     \item In section \ref{sec:related_work} related work, rephrased the part about applicability of distance-based and pattern-based techniques to streaming time-series. 
%     \item Removed claim that we are evaluating unsupervised deep learning algorithms. Added clarification that DAGMM and OC-SVM are unsupervised algorithms, but we evaluate in the semi-supervised setting only in section \ref{sec: predefined-scoring}. 
%     \item In section \ref{sec: scoring} Scoring functions, reworded the description of Gauss-S, addressing the question of small training errors. Also added a line in description of Gauss-D-K to add intuition about the method. 
%     \item Figure 4 has been enlarged but broken down into two parts. Instead of covering all 7 datasets, the figure covers 4 datasets and additional datasets have been moved to SI Fig. S6. 
% \end{itemize}


==> tables/fc_scores_metrics.tex <==
\begin{table}[h]
\centering
\caption{Metrics for predicted labels shown in Fig. \ref{fig:example_scores}}
\label{tab: metrics_example_scores}
\begin{tabular}{lrrr}
\toprule
$\hat{y}$ & $F_1$ &  $p.a. F_1$ &  $Fc_1$ \\
\midrule
$\hat{y}_1$ &        0.2143 &           0.4444 &        0.2553 \\
$\hat{y}_2$ &        0.3333 &           0.3182 &        0.3333 \\
$\hat{y}_3$ &        0.0769 &           0.7368 &        0.1667 \\
$\hat{y}_4$ &        0.6957 &           0.8085 &        0.6667 \\
$\hat{y}_5$ &        0.2286 &           0.9825 &        0.8889 \\
$\hat{y}_6$ &        0.6364 &           1.0000 &        1.0000 \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table}
%   \begin{minipage}[t]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/example_scores_new.pdf}%
%     \caption
%       {%
%         Image of a duck%
%         \label{fig:duck}%
%       }%
%   \end{minipage}\hfill
%   \begin{minipage}[t]{.46\linewidth}
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{lrrr}
%         \toprule
%         $\hat{y}$ & $F_1$ &  $p.a. F_1$ &  $Fc_1$ \\
%         \midrule
%         $\hat{y}_1$ &        0.2143 &           0.4444 &        0.2553 \\
%         $\hat{y}_2$ &        0.3333 &           0.3182 &        0.3333 \\
%         $\hat{y}_3$ &        0.0769 &           0.7368 &        0.1667 \\
%         $\hat{y}_4$ &        0.6957 &           0.8085 &        0.6667 \\
%         $\hat{y}_5$ &        0.2286 &           0.9825 &        0.8889 \\
%         $\hat{y}_6$ &        0.6364 &           1.0000 &        1.0000 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \captionof{table}
%       {%
%         Different kinds of ducks%
%         \label{tab:duck}%
%       }
%   \end{minipage}
% \end{table}


==> tables/omni_pa.tex <==
\begin{table}[]
\caption{Results for $F1_{best}$ for the Omnianomaly algorithm and others with point adjust, averaged over 5 seeds. \agcomment{modify table to show all 3 metrics for SWaT, WADI and SMD.}}
\label{tab: omni-point-adjust}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l|l|rrr@{}}
\toprule
Model                             & Score   & MSL    & SMAP   & SMD    \\ \midrule
UAE             & Gauss-S & 0.9444 & \textbf{0.962}  & 0.9304 \\
NASA LSTM              & Gauss-S & \textbf{0.9744} & 0.9602 & 0.8306 \\
FC AE                    & Gauss-S & 0.8827 & 0.8865 & 0.9395 \\
LSTM AE                  & Gauss-S & 0.8634 & 0.8509 & 0.8879 \\
OmniAnoAlgo (reproduced by us)    & base    & 0.8459 & 0.8678 & 0.9424 \\ 
OmniAnoAlgo (reported by authors) & base    & 0.8535 & 0.9014 & \textbf{0.962}  \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/pre_rec_topk.tex <==
% \begin{landscape}
\begin{table*}[h]
\centering
\caption{Time-wise Precision, $prec_t$, event-wise recall, $rec_e$ and composite F-score $Fc_1$ score for \textit{single-entity} datasets with the \textit{top-k} threshold and \textit{Gauss-D} scoring function, except for starred algorithms.}
\label{tab:pr_rec_single}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|rrr|rrr|rrr}
\toprule
Algo & \multicolumn{3}{c|}{DAMADICS} & \multicolumn{3}{c|}{SWaT} & \multicolumn{3}{c|}{WADI} \\
{} & $prec_t$ & $rec_e$ &  $Fc_1$ & $prec_t$ & $rec_e$ &  $Fc_1$ & $prec_t$ & $rec_e$ &  $Fc_1$ \\
\midrule
DAGMM*                 &   0.0000 &  0.0000 &  0.0000 &   0.0000 &  0.0000 &  0.0000 &   0.0232 &  0.0286 &  0.0256 \\
FC AE        &   0.4186 &  0.6589 &  0.5116 &   0.3051 &  0.5943 &  0.4032 &   0.3888 &  0.9286 &  0.5481 \\
LSTM AE      &   0.4514 &  0.8942 &  0.5999 &   0.3774 &  0.8171 &  0.5163 &   0.2927 &  0.7857 &  0.4265 \\
LSTM VAE              &   0.4456 &  0.8824 &  0.5921 &   0.3079 &  0.8457 &  0.4510 &   0.4043 &  0.9572 &  0.5683 \\
NASA LSTM             &   0.0884 &  0.2353 &  0.1284 &   0.0978 &  0.2629 &  0.1403 &   0.0656 &  0.3143 &  0.1058 \\
OmniAnomaly*           &   0.1064 &  0.2823 &  0.1425 &   0.1044 &  0.2800 &  0.1466 &   0.1695 &  0.4428 &  0.2443 \\
PCA                   &   0.3828 &  0.8824 &  0.5339 &   0.3912 &  0.8286 &  0.5314 &   0.2644 &  0.6429 &  0.3747 \\
Raw Signal            &   0.3515 &  0.8235 &  0.4927 &   0.3009 &  0.5143 &  0.3796 &   0.2869 &  0.7143 &  0.4094 \\
TCN AE       &   0.4629 &  0.8824 &  0.6071 &   0.3596 &  0.6971 &  0.4732 &   \textbf{0.4077} &  0.9714 &  \textbf{0.5741} \\
UAE &   \textbf{0.4824} &  \textbf{0.9412} &  \textbf{0.6378} &   \textbf{0.4244} &  \textbf{0.8743} &  \textbf{0.5713} &   0.3428 &  \textbf{1.0000} &  0.5105 \\
\bottomrule
\end{tabular}
% }
\end{table*}
% \end{landscape}


\begin{table*}[h]
\centering
\caption{Time-wise Precision, $prec_t$, event-wise recall, $rec_e$ and composite F-score $Fc_1$ score for \textit{multi-entity} datasets with the \textit{top-k} threshold and \textit{Gauss-D} scoring function, except for starred algorithms.}
\label{tab:pr_rec_multi}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|rrr|rrr|rrr}
\toprule
Algo & \multicolumn{3}{c|}{MSL} & \multicolumn{3}{c|}{SMAP} & \multicolumn{3}{c|}{SMD} \\
{} & $prec_t$ & $rec_e$ &  $Fc_1$ & $prec_t$ & $rec_e$ &  $Fc_1$ & $prec_t$ & $rec_e$ &  $Fc_1$ \\
\midrule
DAGMM*                 &   0.0893 &  0.4457 &  0.1360 &   0.1247 &  0.4272 &  0.1681 &   0.0108 &  0.0841 &  0.0187 \\
FC AE        &   0.3181 &  0.8815 &  0.4324 &   0.3125 &  0.9444 &  0.4161 &   0.4028 &  0.9538 &  0.5361 \\
LSTM AE      &   0.3302 &  0.9185 &  0.4481 &   0.3694 &  0.9519 &  0.4536 &   0.3931 &  0.9404 &  0.5273 \\
LSTM VAE              &   0.2832 &  0.8074 &  0.3600 &   0.1847 &  0.9167 &  0.2716 &   0.3972 &  0.9259 &  0.5220 \\
NASA LSTM             &   0.3459 &  \textbf{0.9370} &  0.4715 &   0.3185 &  \textbf{0.9667} &  0.4280 &   0.3711 &  0.5339 &  0.3879 \\
OmniAnomaly*           &   0.3124 &  0.7926 &  0.4120 &   0.3122 &  0.8142 &  0.3767 &   0.3802 &  0.9051 &  0.5002 \\
PCA                   &   0.2825 &  0.9259 &  0.4067 &   0.3113 &  0.8179 &  0.3793 &   0.4115 &  0.9090 &  0.5344 \\
Raw Signal            &   0.1831 &  0.5926 &  0.2453 &   0.2028 &  0.5864 &  0.2707 &   0.3770 &  0.9695 &  0.5151 \\
TCN AE       &   0.3253 &  0.8778 &  0.4308 &   0.2945 &  0.9333 &  0.3884 &   \textbf{0.4506} &  0.9678 &  \textbf{0.5844} \\
UAE &   \textbf{0.3998} &  \textbf{0.9370} &  \textbf{0.5111} &   \textbf{0.3727} &  0.9506 &  \textbf{0.4793} &   0.4051 &  \textbf{0.9782} &  0.5501 \\
\bottomrule
\end{tabular}
% }
\end{table*}

==> tables/prec_rec_unsup.tex <==
\begin{table*}[h]
\centering
\setlength{\tabcolsep}{4pt}
\caption{Time-wise Precision, $prec_t$, event-wise recall, $rec_e$, composite F-score $Fc_1$, and the chosen value of $-\log(\epsilon)$ for \textit{single-entity} datasets. Refer to Table \ref{tab: fscore unsup} for key to * symbols. 
} 
\label{tab: pr_rec_unsup}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l|rrrc|rrrc|rrrc}
\toprule
Algo & \multicolumn{4}{c|}{DAMADICS} & \multicolumn{4}{c|}{SWaT} & \multicolumn{4}{c}{WADI} \\
{} & $prec_t$ & $rec_e$ &  $Fc_1$ & $-\log(\epsilon)$ & $prec_t$ & $rec_e$ &  $Fc_1$ & $-\log(\epsilon)$ & $prec_t$ & $rec_e$ &  $Fc_1$ & $-\log(\epsilon)$ \\
\midrule
DAGMM*                    &   0.0000 &  0.0000 &  0.0000 &    5 &   0.0000 &  0.0000 &  0.0000 &    1 &   0.0000 &  0.0000 &  0.0000 &    5 \\
FC AE        &   0.5244 &  0.6118 &  0.5645 &    5 &   0.4909 &  0.4571 &  0.4734 &    4 &   0.5402 &  0.7714 &  \textbf{0.6351} &    5 \\
LSTM AE      &   0.2287 &  0.9412 &  0.3679 &    5 &   0.4934 &  0.7372 &  0.5903 &    5 &   0.2878 &  0.7857 &  0.4212 &    5 \\
LSTM VAE              &   0.5146 &  0.8353 &  0.6365 &    5 &   0.7570 &  0.3828 &  0.5083 &    5 &   0.4319 &  0.8286 &  0.5675 &    3 \\
NASA LSTM             &   0.0700 &  0.2941 &  0.1130 &    5 &   0.2149 &  0.2171 &  0.2085 &    2 &   0.9562 &  0.1286 &  0.2252 &    5 \\
NASA LSTM NPT**                &   0.1859 &  0.1176 &  0.1440 &      &   0.0198 &  0.0400 &  0.0257 &      &   1.0000 &  0.0714 &  0.1333 &      \\
OC-SVM***                   &   0.0171 &  1.0000 &  0.0337 &      &   0.0399 &  0.9143 &  0.0765 &      &   0.1044 &  0.9286 &  0.1876 &      \\
OmniAnomaly*              &   0.0287 &  0.8941 &  0.0557 &    1 &   0.0870 &  0.5829 &  0.1497 &    5 &   0.0574 &  0.8143 &  0.1072 &    1 \\
PCA                   &   0.1445 &  0.9412 &  0.2505 &    5 &   0.5003 &  0.7429 &  0.5979 &    5 &   0.2188 &  0.7143 &  0.3349 &    5 \\
Raw Signal            &   0.5202 &  0.7647 &  0.6192 &    2 &   0.5645 &  0.3429 &  0.4266 &    4 &   0.3868 &  0.5714 &  0.4613 &    3 \\
TCN AE       &   0.4470 &  0.8824 &  0.5927 &    5 &   0.6664 &  0.5828 &  0.6205 &    5 &   0.4476 &  0.9286 &  0.6016 &    3 \\
UAE &   0.4948 &  0.9177 &  \textbf{0.6429} &    5 &   0.5259 &  0.8400 &  \textbf{0.6467} &    5 &   0.3578 &  1.0000 &  0.5267 &    3 \\
\bottomrule
\end{tabular}
% }
\end{table*}

\begin{table*}[]
\centering
\setlength{\tabcolsep}{4pt}
\caption{Time-wise Precision, $prec_t$, event-wise recall, $rec_e$, composite F-score $Fc_1$, and the chosen value of $-\log(\epsilon)$ for \textit{multi-entity} datasets. Refer to Table \ref{tab: fscore unsup} for key to * symbols. 
} 
\label{tab: pr_rec_unsup}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l|rrrc|rrrc|rrrc}
\toprule
Algo & \multicolumn{4}{c|}{MSL} & \multicolumn{4}{c|}{SMAP} & \multicolumn{4}{c}{SMD} \\
{} & $prec_t$ & $rec_e$ &  $Fc_1$ & $-\log(\epsilon)$ & $prec_t$ & $rec_e$ &  $Fc_1$ & $-\log(\epsilon)$ & $prec_t$ & $rec_e$ &  $Fc_1$ & $-\log(\epsilon)$ \\
\midrule
DAGMM*                    &   0.1155 &  0.7506 &  0.1800 &                 1 &   0.1876 &  0.7889 &  0.2419 &                 2 &   0.0000 &  0.0000 &  0.0000 &                 5 \\
FC AE        &   0.3012 &  0.8136 &  0.3947 &                 5 &   0.3219 &  0.9518 &  0.4128 &                 5 &   0.5440 &  0.9318 &  0.6446 &                 5 \\
LSTM AE      &   0.3018 &  0.9148 &  0.4004 &                 5 &   0.3487 &  0.9815 &  0.4276 &                 5 &   0.3139 &  0.9632 &  0.4398 &                 5 \\
LSTM VAE              &   0.2844 &  0.5185 &  0.3230 &                 5 &   0.3090 &  0.7926 &  0.3671 &                 5 &   0.5698 &  0.7948 &  0.6109 &                 5 \\
NASA LSTM             &   0.3290 &  0.9407 &  0.4495 &                 5 &   0.3511 &  0.9914 &  0.4410 &                 5 &   0.3989 &  0.5098 &  0.3336 &                 5 \\
NASA LSTM NPT**                &   0.2833 &  0.5679 &  0.3403 &                   &   0.5139 &  0.8185 &  \textbf{0.5869} &                   &   0.3573 &  0.2298 &  0.1957 &                   \\
OC-SVM***                   &   0.1103 &  0.7593 &  0.1717 &                   &   0.1283 &  0.8549 &  0.1757 &                   &   0.0491 &  0.8726 &  0.0893 &                   \\
OmniAnomaly*              &   0.4236 &  0.9259 &  \textbf{0.5008} &                 1 &   0.4170 &  0.7982 &  0.4542 &                 2 &   0.3805 &  0.9058 &  0.4444 &                 5 \\
PCA                   &   0.2578 &  0.8827 &  0.3527 &                 5 &   0.3103 &  0.8117 &  0.3638 &                 5 &   0.3785 &  0.9084 &  0.4915 &                 5 \\
Raw Signal            &   0.2286 &  0.4444 &  0.2618 &                 4 &   0.2593 &  0.4691 &  0.2924 &                 5 &   0.5965 &  0.9292 &  \textbf{0.6952} &                 5 \\
TCN AE       &   0.3711 &  0.7630 &  0.4406 &                 5 &   0.3779 &  0.9204 &  0.4470 &                 5 &   0.4798 &  0.9654 &  0.5990 &                 5 \\
UAE &   0.3692 &  0.8568 &  0.4571 &                 5 &   0.4273 &  0.9580 &  0.5135 &                 5 &   0.4093 &  0.9690 &  0.5440 &                 5 \\
\bottomrule
\end{tabular}
% }
\end{table*}
